Approximate Nearest Neighbor Search on High Dimensional Data --- Experiments, Analyses, and Improvement (v1.0)

Approximate Nearest neighbor search (ANNS) is fundamental and essential operation in applications from many domains, such as databases, machine learning, multimedia, and computer vision. Although many algorithms have been continuously proposed in the literature in the above domains each year, there is no comprehensive evaluation and analysis of their performances. In this paper, we conduct a comprehensive experimental evaluation of many state-of-the-art methods for approximate nearest neighbor search. Our study (1) is cross-disciplinary (i.e., including 16 algorithms in different domains, and from practitioners) and (2) has evaluated a diverse range of settings, including 20 datasets, several evaluation metrics, and different query workloads. The experimental results are carefully reported and analyzed to understand the performance results. Furthermore, we propose a new method that achieves both high query efficiency and high recall empirically on majority of the datasets under a wide range of settings.

==> algs-Space.tex <==
\section{Space Partitioning-based Methods}
\label{sec:algs_tree}
%% neighbor in high dim space is still neighbor in low dim space
%%
Methods in this category can be deemed as dividing the entire high dimensional
space into multiple disjoint regions. Let the query $q$ be located in a region
$r_q$, then its nearest neighbors should reside in $r_q$ or regions
%\emph{surrounding} $r_Q$. % %% or just mention close to $r_Q$?
\emph{near} $r_q$. % %% or just mention close to $r_Q$?
The major difference with the LSH-based methods is that methods in this category
typically make use of the data distributions to achieve higher efficiency, at
the cost of relinquishing the theoretical guarantees.

% Not all partitioning methods are valid here. A valid method needs to support
% efficient, $o(n)$, methods to locate $r_Q$. It is also desirable that we can
% enumerate surrounding regions of $r_Q$, although this is not strictly necessary
% as we can also compensate that using multiple space partitioning methods.
% %% e.g., hierarchical clustering does not satisfy this condition. What about
% %% spectral clustering (it satisifies, as it is just a linear projection and
% %% then quantization, so both locating and enumerating can be done.


The representative space partitioning methods are \Algkmeans{} (most tree-based
methods and PQ~\cite{DBLP:journals/pami/JegouDS11}), order-$k$ voronoi diagrams
(e.g., \AlgNAPP{}~\cite{DBLP:journals/pvldb/NaidanBN15}), and spectral
clustering (e.g., AGH~\cite{DBLP:conf/icml/LiuWKC11}). %
Due to the large number of algorithms in this category, we further categorized
them into \emph{encoding-based} methods and \emph{tree-based} methods.

%\subsection{Data-sensitive hashing methods}
%\label{subsec:lhash}


\subsection{Encoding-based Methods}
\label{subsec:lhash}

A large body of works have been dedicated to learning hash functions from the
data distribution so that the nearest neighbor search result in the hash coding
space is as close to the search result in the original space as possible. Please
refer to~\cite{DBLP:journals/corr/WangSSJ14,DBLP:journals/pieee/WangLKC16} for a
comprehensive survey.

Some example methods we evaluated in this category include Neighbor Sensitive
Hashing~\cite{DBLP:journals/pvldb/ParkCM15}, Selective
Hashing~\cite{DBLP:conf/kdd/GaoJOW15}, Anchor Graph
Hashing~\cite{DBLP:conf/icml/LiuWKC11}, Scalable Graph
Hashing~\cite{DBLP:conf/ijcai/JiangL15}, Neighborhood APProximation index~\cite{DBLP:journals/pvldb/NaidanBN15}, and Optimal Product
Quantization \cite{DBLP:journals/pami/GeHK014}.


The Optimal Product Quantization (\AlgOPQ) method is chosen as the
representative of this category due to its popularity and good performance in
practice. Meanwhile, we also evaluate other representative data-sensitive
hashing methods including Spectral Hashing~\cite{DBLP:conf/nips/WeissTF08}, ICA
hashing~\cite{DBLP:conf/cvpr/HeCRB11}, %
% Kernelized spectral hashing~\cite{DBLP:conf/iccv/KulisG09},
weighted hashing~\cite{DBLP:conf/cikm/WangZS13}, PCA hashing
\cite{DBLP:conf/psivt/MatsushitaW09}, anchor graph hashing
\cite{DBLP:conf/icml/LiuWKC11} and scalable Graph
hashing~\cite{DBLP:conf/ijcai/JiangL15}.

We exclude a recent work~\cite{DBLP:journals/pvldb/AndreKS15} optimizing the
performance of product quantization-based method as it is mainly based on
utilizing the hardware-specific features.

%\subsubsection{Spectral Hashing}
%
%spectral hashing aims to find an easy-evaluated hash function satisfying two requirements: bit balance and bit uncorrelation. Rather than solving the above problem directly, a simple approximate solution with the assumption of uniformly data distribution is used. The algorithm is given as follows:
%\begin{itemize}
%\item Find the principal components of the $N$ $d$-dimensional reference data items using principal component analysis (PCA).
%\item Compute the $M$ 1D Laplacian eigenfunctions with the smallest eigenvalues along each PCA direction.
% \item Pick the $M$ eigenfunctions with the smallest eigenvalues among $Md$ eigenfunctions.
%\item Threshold the eigenfunction at zero, obtaining the binary codes.
%\end{itemize}

\subsubsection{Anchor Graph Hashing}

Hashing with graphs\cite{DBLP:conf/icml/LiuWKC11} uses the anchor graph to approximate the neighborhood graph and accordingly uses the graph Laplacian over the anchor graph to approximate the graph Laplacian of the original graph for fast computing the eigenvectors with a side contribution of exploiting a hierarchical hashing to address the boundary issue.


%\myparagraph{Scalable Graph hashing}





\subsubsection{Neighbor Sensitive Hashing}

For hashing-based methods, the accuracy is judged by their effectiveness in preserving the kNN relationships (among the original items) in the Hamming space. That is, the goal of the optimal hash functions is that the relative distance of the original items are ideally linear to relative Hamming distance. To preserve the original distances, existing hashing techniques tend to place the separators uniformly, while those are more effective for rNN searching.

Given a reference point $p$, NSH changes the shape of the projection function which impose a larger slope when the original distance to $p$ is small, and allow the projection distance to remain stable beyond a certain distance. Hence, when using the traditional function under the projection space, it is more likely to be assigned with different hash codes for the points close to $p$. If the distances between the query $q$ and $p$ is smaller than a threshold, the above property also apply to $q$. For handling all possible queries, NSH selects multiple pivots and limits the maximal average distances between a pivot and its closest neighbor pivot to ensure that there will be at least one nearby pivot for any novel query.

\subsubsection{NAPP}
permutation methods are dimensionality-reduction approaches, which assess similarity of objects based on their relative distances to some selected reference points, rather than the real distance values directly. An advantage of permutation methods is that they are not relying on metric properties of the original distance and can be successfully applied to non-metric spaces.
%
The underpinning assumption of permutation methods is that most nearest neighbors can be found by retrieving a small fraction of data points whose pivot rankings are similar to the pivot ranking of
the query.

A basic version of permutation methods select $m$ pivots $\Pi_{i}$ randomly from the data points. For each data point $x$, the pivots are arranged in the order of increasing distance from $x$. Such a permutation of pivots is essentially a low-dimensional integer-valued vector whose $i$-th element is the ranking order of the $i$-th pivot in the set of pivots sorted by their distances from $x$. For the pivot closest to the data point, the value of the vector element is one, while for the most distance pivot the value is $m$.

In the searching step, a certain number of candidate points are retrieved whose permutations are sufficiently close to the permutation of the query vector. Afterwards, the search method sort these candidate data points based on the original distance function.

This basic method was improved in several ways. For example, one can index permutations rather than searching them sequentially: It is possible to employ a permutation prefix tree, an inverted
index, or an index designed for metric spaces, e.g., a VPtree.

In this paper, we use the implementation by Bilegsaikhan. First, they also select $m$ pivots and compute the permutations induced by data points. For each data point, $m_{i} \le m$ most closest pivots are indexed in a inverted file. At query time, the data points that share at least $t$ nearest neighbor pivots with the query are selected. Then, these candidates points are compared directly against the query based on the real distance.

\subsubsection{Selective LSH}

LSH is designed for finding points within a fixed radius of the query point, which is more suitable for radius search. For a k-NN problem, the corresponding radii for different query points may vary by orders of magnitude, depending on the local density around the query point. Selective Hashing is especially suitable for k-NN search which create multiple LSH indices with different granularities (radii). Then, every data object is only stored in one selected index. Data points in dense regions are stored in the index with small granularity, while data points in sparse regions are stored in the index with large granularity. Hence, there is almost no extra storage overhead compared with one fixed radius. Using this idea, selective hashing method achieves good quality for k-NN search and avoid visiting multiple indices. In the querying phase, the algorithm will push down the query and check the cell with suitable granularity.


\subsubsection{Optimal Product Quantization (\AlgOPQ)}
\label{subsubsec:opq}

Vector quantization (VQ)~\cite{DBLP:journals/tit/GrayN98} is a popular and
successful method for ANN search, which could be used to build inverted index
for non-exhaustive search. A vector $x \in \mathbb{R}^d$ is mapped to a codeword
$\mathbf{c}$ in a \emph{codebook} $\mathbf{C}=\set{ \mathbf{c}_j }$ with $i$ in
a finite index set. The mapping, termed as a \emph{quantizer}, is denoted by:
$x \rightarrow \mathbf{c}(i(x))$, where the function $i(\cdot)$ and
$\mathbf{c}(\cdot)$ is called \emph{encoder} and \emph{decoder}, respectively.
The $k$-means approach has been widely used to construct the codebook
$\mathbf{C}$ where $i(x)$ is the index of the nearest \emph{mean} of $x$ and
$\mathbf{c}(i(x))$ is corresponding \emph{mean}. %\fixme{???} %
An inverted index can be subsequently built to return all data vectors that are
mapped to the same codeword.

A product quantizer~\cite{DBLP:journals/pami/JegouDS11} is a solution to VQ when
a large number of codewords are desired. The key idea is to decompose the
original vector space into the Cartesian product of $M$ lower dimensional
subspaces and quantize each subspace separately. Suppose $M=2$ and the
dimensions are evenly partitioned. Each vector $x$ can be represented as the
concatenation of $2$ sub-vectors: $[x^{(1)}, x^{(2)}]$, Then we have
$\mathbf{C} = \mathbf{C^{(1)}} \times \mathbf{C^{(2)}}$ where $\mathbf{C}^{(1)}$
(resp.\ $\mathbf{C}^{(2)}$) is constructed by applying the $k$-means algorithm
on the subspace consisting of the first (resp.\ second) half dimensions. As
such, there are $k \times k$ codewords, and $x$'s nearest codeword $\mathbf{c}$
in $\mathbf{C}$ is the concatenation of the two nearest sub-codewords $c^{(1)}$
and $c^{(2)}$ based on its sub-vectors $x^{(1)}$ and $x^{(2)}$, respectively.
Given a query vector $q = [q^{(1)}, q^{(2)}]$, the search algorithm
in~\cite{DBLP:conf/cvpr/BabenkoL12} first retrieves $L$ closest sub-codedwords
$\set{\mathbf{C^{i}_j}}_{i \in \set{1, 2}, j \in \set{1, 2, \ldots L}}$ in each
subspaces based on $q^{(1)}$ and $q^{(2)}$, respectively, and then a multi-sequence algorithm based on a priority queue is applied to traverse the set of pairs $\set{\mathbf{C^{1}_j},\mathbf{C^{2}_j}}$ in increasing distance to achieve candidate codeword set $\mathcal{C}$, finally, the distances
of points belonging to one of the code word in $\mathcal{C}$ are examined via the inverted
index.

%compute the $L \times L$ candidate codeword set $\mathcal{C}$,
% explores $L\times L$
% possible codewords in $\mathbf{C^1}\times\mathbf{C^2}$ to identify the kNN.

Recently, the Optimal Product Quantization (\AlgOPQ) method is
proposed~\cite{DBLP:journals/pami/GeHK014}, which optimizes the index by
minimizing the quantization distortion with respect to the space decompositions
and the quantization codewords.


\subsection{Tree-based Space Partition Methods}
\label{subsec:tree}

Tree-based space partition has been widely used for the problem of exact and
approximate NNS. Generally, the space is partitioned in a hierarchically manner
and there are two main partitioning schemes: \textit{pivoting} and
\textit{compact} partitioning schemes.
% Pivoting methods partition the vector space relying on the distance from the data point to pivots
% while compact partitioning methods either divide the data points into clusters, approximate Voronoi partitions or random divided space.
In this subsection, we introduce two representative compact partitioning
methods, \Algannoy~\cite{misc:url/annoy} and
\Algflann~\cite{DBLP:journals/pami/MujaL14}.
as they are used in a commercial recommendation system and widely used in the
Machine Learning and Computer Vision communities. In addition, we also evaluate
a classical pivoting partitioning method, \textit{Vantage-Point}
tree~\cite{DBLP:conf/soda/Yianilos93} (VP-tree), in the experiments.

%\subsubsection{Tree-based Space Partition Methods}
%\label{subsec:tree}
%
%ree-based space partition has been widely used for exact and
%approximate NNS in low dimensional space. %
%% While many of the straight-forward
%% generalization to high-dimensional space do not work, there are
%It can be modified to work for approximate NNS in high-dimensional space.
%%
%%
%% Generally, the space is partitioned in a hierarchically manner
%% and there are two main partitioning schemes: \textit{pivoting} and
%% \textit{compact} partitioning schemes.
%% Pivoting methods partition the vector space relying on the distance from the data point to pivots
%% while compact partitioning methods either divide the data points into clusters, approximate Voronoi partitions or random divided space.
%In this subsection, we introduce three methods implemented in two systems,
%\Algflann~\cite{DBLP:journals/pami/MujaL14} and
%\Algannoy~\cite{misc:url/annoy}.
%% Both of them have been widely used in a
%% commercial recommendation system or in the Machine Learning and Computer Vision
%% communities, and achieve competative performance.
%The three methods belong to two subcategories: axis-parallel hyperplane-based, and
%hierarchical \Algkmeans{}-based. In our experimental evaluation, we also include
%an improved \textit{Vantage-Point} (VP) tree~\cite{DBLP:conf/soda/Yianilos93}.



\subsubsection{\Algflann}
\label{subsubsec:flann}

\Algflann is an automatic nearest neighbor algorithm configuration method which
select the most suitable algorithm from \textit{randomized
  kd-tree}~\cite{DBLP:conf/cvpr/Silpa-AnanH08}, \textit{hierarchical k-means
  tree}~\cite{DBLP:journals/tc/FukunagaN75}\footnote{Also known as
  GNAT~\cite{DBLP:conf/vldb/Brin95} and vocabulary
  tree~\cite{DBLP:conf/cvpr/SchindlerBS07}.}, and \textit{linear scan} methods
for a particular data set. Below, we briefly introduce the two modified
tree-based methods and the algorithm selection criteria of \Algflann based
on~\cite{DBLP:journals/pami/MujaL14} and Version~1.8.4 source code.
%%%!! 1) as \cite{DBLP:conf/cvpr/SchindlerBS07} puts it, hierarchical k-means tree
%%%   can be thought of as a hierarchical Voronoi diagram.
%%%   2) \cite{DBLP:journals/tc/FukunagaN75} uses branch-and-bound (or called
%%%   best-bin-first by \cite{DBLP:conf/cvpr/SchindlerBS07}).
%%%   \cite{DBLP:conf/cvpr/SchindlerBS07} proposes an alternative search
%%%   strategy: it considers all surviving level-i nodes in each iteration, and
%%%   keeps only l best level-i nodes alive.


\myparagraph{Randomized kd-trees}%

The main differences from \Algflann{}'s randomize kd-trees with the traditional
kd-tree are:
\begin{inparaenum}[(i)]
\item The data points are recursively split into two halfs by first choosing a
  splitting dimension and then use the perpendicular hyperplane centered at the
  \emph{mean} of the dimension values of all input data points.
\item The splitting dimension is chosen at random from top-5 dimensions that
  have the largest sample variance based on the input data points.
\item Multiple randomized kd-trees are built as the index.
\item To answer a query $q$, a depth-first search prioritized by some heuristic
  scoring function are used to search multiple randomized
  kd-trees with a shared priority queue and candidate result set.
  The scoring function always favors the child node that is closer to the query
  point, and


% below a threshold $b$. When searching the randomized kd-forest, a single
% priority queue is maintained across all the randomized trees. The priority queue
% is ordered by increasing distance to the decision boundary of each branch in the
% queue.
% % , so the search will first explore the closest leaves from all the trees.


  lower bounding distance
 is maintained across all the randomized trees. The priority queue
% is ordered by increasing distance to the decision boundary of each branch in the
% queue.

\end{inparaenum}



% are proposed in~\cite{DBLP:conf/cvpr/Silpa-AnanH08} that modify the traditional
% kd-trees for high dimensional data. The algorithm recursively split the data
% evenly based on a chosen dimension, where \fixme{check flann}
% %
% %
% nearest-neighbor search. The randomized kd-tree building process starts with all
% the points in the dataset and splits the them on the dimension which is chosen
% randomly from the top $p$ dimensions with the highest variance, where variances
% of each tree are computed based on different samples.\fixme{why different
%   samples?} %
% Then the algorithm recursively repeats the partitioning for each of the
% partitioning results and stops when the number of points in each node falls
% below a threshold $b$. When searching the randomized kd-forest, a single
% priority queue is maintained across all the randomized trees. The priority queue
% is ordered by increasing distance to the decision boundary of each branch in the
% queue.
% % , so the search will first explore the closest leaves from all the trees.

\myparagraph{Hierarchical k-means tree}%
is constructed by partitioning the data points at each level into $K$ regions
using K-means clustering. Then the same method is applied recursively to the
data points in each region. The recursion is stopped when the number of points
in each leaf node is smaller than $K$. The tree is searched by initially
traversing the tree from the root to the closest leaf, during which the
algorithm always picks up the the inner node closest to the query point, and
adding all unexplored branches along the path to a priority queue.

% The priority queue is sorted in increasing distance from the query point to
% the boundary of the branch being added to the queue. After the initial tree
% traversal, the algorithm resumes traversing the tree, always starting with the
% top branch in the queue.

\myparagraph{\Algflann}%
carefully chooses one of the three candidate algorithms by minimizing a cost
function which is a combination of the search time, index building time and
memory overhead to determine the search algorithm. It uses cross-validation
using random sub-samples to generate the data and the query points for the
optimization.


\subsubsection{\Algannoy}
\label{subsubsec:annoy}

\Algannoy is an empirically engineered algorithm that has been used in the
recommendation engine in \url{spotify.com}, and has been recognized as one of
the best \ANN{} libraries.
% mainly based on the random
% projection (RP) trees~\cite{DBLP:conf/stoc/DasguptaF08}.

\myparagraph{Index Construction}. %

In earlier versions, \Algannoy{} constructs multiple random projection
trees~\cite{DBLP:conf/stoc/DasguptaF08}. In the latest version (as of March
2016), it instead constructs multiple hierarchical 2-means trees. %
Each tree is independently constructed by recursively partitioning the data
points as follows. At each iteration, two centers are formed by running a
simplified clustering algorithm on a subset of samples from the input data
points. The two centers defines a partition hyperplane which has equidistant
from the centers. Then the data points are partitioned into two sub-trees by the
hyperplane, and the algorithm builds the index on each sub-trees recursively.
% The partitioning stops when the number of points in each leaf node falls below
% $d+2$. % where $d$ is the dimensionality of the data.

\myparagraph{Search}. %

The search process is carried out by traveling tree nodes of the multiple RP
trees. Initially, the roots of the RP trees are pushed into a maximum priority
queue with key values infinity. For a given tree node $n_i$ with parent node
$n_p$, if the query $q$ falls into the subtree of $n_i$, the key of $n_i$ is the
minimum of its parent node and the distance to the hyperplane; otherwise, the
key is the minimum of its parent node and the negative value of the distance to
the hyperplane. At each iteration, the node with the maximum key is chosen for
exploration.%\fixme{double check index and search. Selecting random projections
 % vs random pair of points? LB distance? }




\subsubsection{VP-Tree}

VP-tree is a classic space decomposition tree that recursively divides the space with respect to a randomly chosen pivot $\pi$. For each partition, a median value R of the distance from $\pi$ to every other point in the current partition was computed. The pivot-centered ball with the radius $R$ is used to partition the space: the inner points are placed into the left subtree, while the outer points are placed into the right subtree (points that are exactly at distance $R$ from $\pi$ can be placed arbitrarily). Partitioning stops when the number of points falls below the threshold $b$.

In classic VP-tree, the triangle inequality can be used to prune unpromising partitions as follows: imagine that $r$ is a radius of the query and the query point is inside the pivot-centered ball (i.e., in the left subtree). If $R - d(\pi,q) > r$, the right partition cannot have an answer and the right subtree can be safely pruned. The nearest-neighbor search is simulated as a range search with a decreasing radius: Each time we evaluate the distance between $q$ and a data point, we compare this distance with $r$. If the distance is smaller, it becomes a new value of $r$. In \cite{DBLP:journals/pvldb/NaidanBN15}, a simple polynomial pruner is employed. More specifically, the right partition can be pruned if the query is in the left partition and $(R-d(\pi,q))^{\beta}\alpha_{left} > r$. The left partition can be pruned if the query is in the right partition and $(d(\pi,q)-R)^{\beta}\alpha_{left} > r$.


